Low energy excitations of vector spin glasses

The work of this thesis concerns the problem of linear low energy excitations of vector spin glass models. An analytical and numerical study is carried out, considering a fully connected random-field Heisenberg model at zero temperature, a fully-connected vector p-spin glass model and a sparse random-field Heisenberg model. We test these models against the low temperature behavior of finite dimensional glassy systems, in particular we show that they posses phases where the density of states is gapless with quasi-localised modes. In the case of the sparse model, we show that the density of states follows a quartic law at low frequency, consistently with several recent measures of this quantity that can be found in the literature of computer glasses. In all the three models, the spin glass transition is characterised in terms of the behavior of the softest excitations. We found that in the fully connected models the zero temperature spin glass transition in a field is a delocalisation transition of the softest modes. In the sparse case, a weaker form of delocalisation appears at the transition. These results broaden our understanding of the zero temperature critical point, by showing how spin glass ordering affects the way the system responds to small magnetic perturbations.

==> Equation_breaking_point.tex <==
\chapter{Derivation of the breaking point equation}
\label{sec:break_point_eq}

==> FP.tex <==
%%%%%%%%%%%%%

In order to compute the Glassy Potential given by formula (ref), we use the Replica Trick and rewrite the logarithm; then, using the self-averaging property we average separately numerator and denominator:
\begin{eqnarray*}
  & \frac{\overline{\underset{\{\boldsymbol{S}_1\}}{\sum}\exp\left\{-\beta_0H_1[\boldsymbol{S}_1]\right\}\ln Z_J^{(1)}(\boldsymbol{S}_1|r, \beta_0, q, \beta)}}{\overline{\underset{\{\boldsymbol{S}\}}{\sum}e^{-\beta_0 H[\boldsymbol{S}]}}}\,=\, \\
   & e^{-\frac{N\beta_0^2f(1)}{2}}\underset{m\rightarrow 0}{\lim}\,\frac{\underset{\{\boldsymbol{S}_1\}}{\sum}\overline{e^{-\beta_0H_1[\boldsymbol{S}_1]}Z_J^{(1)}(\boldsymbol{S}_1|r, \beta_0, q, \beta)^m}-e^{\frac{N\beta_0^2f(1)}{2}}}{m}
\end{eqnarray*}
where $\underset{\bf S}{\sum}(\cdot)\equiv \overset{N}{\underset{k=1}{\prod}}\,\int d\Vec{S}_k\,\delta(S_k-1)(\cdot)$. After some rearrangements, this last quantity reads
\begin{eqnarray*}
    && -V=\lim_{m\rightarrow 0}\frac{\int\,D\boldsymbol{\hat{Q}}\,\exp\left(+N\,A[\boldsymbol{\hat{Q}}]\right)-1}{m} \\
   && A[\boldsymbol{\hat{Q}}]\,=\,\frac{\beta^2}{2}\sum_{\alpha\beta}\sum_{a,b>1}f(Q_{ab}^{\alpha\beta})+\frac{\beta\beta_0}{2}\sum_{\alpha}\sum_{a>1}f(Q_{1 a}^{\alpha\alpha})\\
    && -i\sum_{\alpha\beta}\sum_{(a b)}\hat{Q}_{a b}^{\alpha\beta}Q_{a b}^{\alpha\beta}-i\sum_{\alpha}\sum_{a>1}\hat{Q}_{1 a}^{\alpha\alpha}Q_{1 a}^{\alpha\alpha}+\ln\zeta(\boldsymbol{\hat{Q}}) \\
    && \zeta(\boldsymbol{\hat{Q}})\,=\,\underset{\{\boldsymbol{S}_1\}}{\sum}\underset{\{\boldsymbol{S}_2^{(1)}\}}{\sum}\dots\underset{\{\boldsymbol{S}_n^{(m)}\}}{\sum}\,\exp\Bigl[i\sum_{\alpha}\sum_a\hat{Q}_{1 a}^{\alpha\alpha}\boldsymbol{S}_1\cdot\boldsymbol{S}_a^{\alpha}+ \\
    && i\sum_{\alpha\beta}\sum_{(ab)}\hat{Q}_{a b}^{\alpha\beta}\boldsymbol{S}_a^{\alpha}\cdot\boldsymbol{S}_b^{\beta}\Bigr]
\end{eqnarray*}
where the greek indices stand for the $m$ replicas, whereas latin indices for the $n$ replicas. One has $Q_{ab}^{\alpha\alpha}\,=\,q$ for $a,b>1$ and $a\neq b$, $Q_{1a}=r$ for $a>1$, $Q_{aa}=1$; as to the non-diagonal elements $Q_{ab}^{\alpha\beta}$, we assume that they are identically zero: this is equivalent to ask that replicas belonging to different $m$ blocks are independent. With this ansatz, one finds that $A$ is proportional to $m$, so that, after performing a saddle point expansion, the limit $m\rightarrow 0$ returns
\begin{eqnarray}
\label{eq:V1}
    && -V\,=\,\frac{1}{2}\sum_{a\neq b}[\beta_a\beta_bf(Q_{ab})-i\hat{Q}_{ab}Q_{ab}] \\
  && \zeta\,=\,\underset{\{\boldsymbol{S}_1\}}{\sum}\dots\underset{\{\boldsymbol{S}_n\}}{\sum}\,\exp\left[i\sum_{(ab)}\hat{Q}_{ab}(\boldsymbol{S}_a\cdot\boldsymbol{S}_b)\right] \\
    && i\hat{Q}_{ab}=\beta_a\beta_bf'(Q_{ab}),\,\,\,a\neq b
\end{eqnarray}
In order to complete the computation, we substitute in $Q_{ab}$ the ansatz previously established, $Q_{1a}=r$ for $a>1$ and $Q_{ab}=q$ for $a\neq b$, and after that we divide V by $n-1$ and $\beta$ and perform the limits $n\rightarrow 1$ and $\beta\rightarrow\infty$. After some manipulations, the term $\ln\zeta$ becomes
\begin{eqnarray*}
& \ln\zeta\,=\,-\frac{n-1}{2}\beta^2f'(q)+\ln[1+ \\
& \frac{n-1}{S_m}e^{-\frac{\beta_0^2f'(r)}{2f'(q)}}\int\,D_{f'(q)}\,\Vec{h}\,Y(\frac{\beta_0f'(r)}{f'(q)}h)\ln Y(\beta h)+O(n-1)^2]\nonumber\\
& \simeq -\frac{n-1}{2}\beta^2f'(q)+\frac{n-1}{S_m}\beta e^{-\frac{\beta_0^2f'(r)}{2f'(q)}}\int\,D_{f'(q)}\,\Vec{h}\,Y\left(\frac{\beta_0f'(r)}{f'(q)}h\right) h
\end{eqnarray*}
where
\begin{eqnarray*}
    && \int D_{\hat{q}}\Vec{h}\,(\cdot)\equiv\int \frac{d\Vec{h}}{(2\pi\hat{q})^{m/2}}\,e^{-\frac{h^2}{2\hat{q}}}\,(\cdot)\nonumber \\
    && S_m\,=\,\int\,d^m\Vec{S}\,\delta(|\Vec{S}|-1)\equiv \frac{2\,\pi^{m/2}}{\Gamma(m/2)} \\
    && Y(x)\,=\,(2\pi)^{m/2}\frac{I_{m/2-1}(x)}{x^{m/2-1}}.
\end{eqnarray*}
The remaining addendum in \eqref{eq:V1} reads
\begin{eqnarray*}
    && \frac{1}{2}\sum_{a\neq b}[\beta_a\beta_bf(Q_{ab})-f'({Q}_{ab})Q_{ab}]\,=\,\\
    && (n-1)\beta_0\beta[f(r)-r\,f'(r)]+\frac{(n-1)(n-2)}{2}\beta^2[f(q)-q\,f'(q)]
\end{eqnarray*}
Putting everything together, we get
\begin{eqnarray*}
    && -\frac{1}{\beta (n-1)}V=\beta_0[f(r)-r f'(r)] \\
    && +\frac{e^{-\frac{\beta_0^2f'(r)}{2f'(q)}}}{S_m} \int\,D_{f'(q)}\,\Vec{h}\,Y\left(\frac{\beta_0f'(r)}{f'(q)}h\right) h \\
    && -\frac{\beta}{2}[f(q)-f(1)+f'(q)(1-q)]
\end{eqnarray*}
The last addendum in the r.h.s. of this last equation is of order $(1-q)^2$ for $\beta\rightarrow\infty$: since $1-q=O(\beta^{-1})$, finally we get for $\beta\rightarrow\infty$
\begin{eqnarray}
    && V_G(\beta_0, r)\,=\,-\beta_0[f(r)-r f'(r)] \\
    && -\frac{e^{-\frac{\beta_0^2f'(r)}{2f'(1)}}}{S_m} \int\,D_{f'(1)}\,\Vec{h}\,Y\left(\frac{\beta_0f'(r)}{f'(1)}h\right) h\nonumber.
\end{eqnarray}


==> Nsite_VS_dist_z=3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1078,704){\makebox(0,0)[r]{\strut{}1E+00}}%
      \put(1078,1390){\makebox(0,0)[r]{\strut{}1E+01}}%
      \put(1078,2076){\makebox(0,0)[r]{\strut{}1E+02}}%
      \put(1078,2762){\makebox(0,0)[r]{\strut{}1E+03}}%
      \put(1078,3447){\makebox(0,0)[r]{\strut{}1E+04}}%
      \put(1078,4133){\makebox(0,0)[r]{\strut{}1E+05}}%
      \put(1078,4819){\makebox(0,0)[r]{\strut{}1E+06}}%
      \put(2142,484){\makebox(0,0){\strut{}$5$}}%
      \put(3307,484){\makebox(0,0){\strut{}$10$}}%
      \put(4473,484){\makebox(0,0){\strut{}$15$}}%
      \put(5638,484){\makebox(0,0){\strut{}$20$}}%
      \put(6803,484){\makebox(0,0){\strut{}$25$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2761){\rotatebox{-270}{\makebox(0,0){\strut{}$\overline{\mathcal{N}(d)}$}}}%
      \put(4006,154){\makebox(0,0){\strut{}$d$}}%
      \csname LTb\endcsname%%
      \put(2314,4666){\makebox(0,0)[r]{\strut{}$N=2^{10}$}}%
      \csname LTb\endcsname%%
      \put(2314,4486){\makebox(0,0)[r]{\strut{}$N=2^{14}$}}%
      \csname LTb\endcsname%%
      \put(2314,4306){\makebox(0,0)[r]{\strut{}$N=2^{16}$}}%
      \csname LTb\endcsname%%
      \put(2314,4126){\makebox(0,0)[r]{\strut{}$N=2^{18}$}}%
      \csname LTb\endcsname%%
      \put(2314,3946){\makebox(0,0)[r]{\strut{}$N=2^{20}$}}%
      \csname LTb\endcsname%%
      \put(2314,3766){\makebox(0,0)[r]{\strut{}$G(d, 2^{10})$}}%
      \csname LTb\endcsname%%
      \put(2314,3586){\makebox(0,0)[r]{\strut{}$G(d, 2^{14})$}}%
      \csname LTb\endcsname%%
      \put(2314,3406){\makebox(0,0)[r]{\strut{}$G(d, 2^{16})$}}%
      \csname LTb\endcsname%%
      \put(2314,3226){\makebox(0,0)[r]{\strut{}$G(d, 2^{18})$}}%
      \csname LTb\endcsname%%
      \put(2314,3046){\makebox(0,0)[r]{\strut{}$G(d, 2^{20})$}}%
      \csname LTb\endcsname%%
      \put(2314,2866){\makebox(0,0)[r]{\strut{}Tree}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Nsite_VS_dist_z=3}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> TAP_Fluctuations_SK.tex <==
\chapter{Longitudinal Fluctuations of TAP Hessian}

With this definition, we can compute easily the distribution function of the $\{\kappa_i\}$
\begin{eqnarray}
\label{eq:pdf_ks}
    && P_k(\kappa)\,=\,\int_0^{\infty}dh\;P_h(h)\;\delta\left(\kappa-\frac{1}{\beta\;g_d'(\beta h)}+\frac{d}{\beta}\right)\, \\
    &&  \nonumber \\
    && =\,\frac{P_h(\frac{1}{\beta}\varphi_d(\beta \kappa+d))g_d^{'}(\varphi_d(\beta \kappa+d))^2}{|g_d^{''}(\varphi_d(\beta \kappa+d))|} \nonumber
\end{eqnarray}
where we have introduced $\varphi_d$, the inverse of $1/g_d^{'}$. In the $d=1$ case, one has
\begin{eqnarray*}
    \frac{1}{g_1'(x)}\,=\,\frac{1}{1-\tanh^2(x)}\qquad \varphi_1(y)\,=\,\operatorname{atanh}\left(\sqrt{1-\frac{1}{y}}\right)
\end{eqnarray*}
\begin{eqnarray*}
    g_1^{''}(\varphi_1(y))\,=\,-\frac{2}{y}\sqrt{1-\frac{1}{y}}\qquad g_1^{'}(\varphi_1(y))\,=\,\frac{1}{y} 
\end{eqnarray*}
\begin{equation}
\label{eq:Pk_1}
    P_k(\kappa)\,=\,\frac{\sqrt{\beta}\;\mathcal{G}_{q+H^2}\left(\frac{1}{\beta}\operatorname{atanh}\left(\sqrt{1-\frac{1}{\beta \kappa+1}}\right)\right)}{(\beta \kappa+1)\sqrt{1-\frac{1}{1+\beta \kappa}}}
\end{equation}
This distribution has the following asymptotic behaviors
\begin{eqnarray}
\label{eq:Pk_asymptotics}
    && P_k(\kappa)\sim \frac{1}{\sqrt{\kappa}}\qquad \kappa\rightarrow 0_ \\
    && P_k(\kappa)\sim \frac{\exp(-\frac{\log^2(\beta \kappa/2)}{2\beta (q+H^2)})}{\sqrt{\beta} \kappa}\qquad \kappa\rightarrow\infty
\end{eqnarray}
As the temperature goes to zero, the tail of the distribution becomes slowly non-integrable: longitudinal excitations go to infinity, as it should be since at zero temperature there are only transverse fluctuations. Clearly this behavior stands equal for any $d$, whereas the behavior close to the origin depends on the value of $d$: while at small temperatures we expect to find the same phenomenology of the $T=0$ spectra we are going soon to study, at higher temperatures
in order not to lengthen to much the discussion, we have left to {\color{red} Appendix (XXXX)} the remaining details. 


==> eigenvector_moments_expansion_edge.tex <==
\chapter{Expansion of eigenvector moments close to the band edges}
\label{sec:stat_eigvec_edges}

blmdslgdsmfldsm
